Eliminating Feature Ambiguity for Few-Shot Segmentation

Recent advancements in few-shot segmentation (FSS) have exploited pixel-by-pixel matching between query and support features, typically based on cross attention, which selectively activate query foreground (FG) features that correspond to the same-class support FG features. However, due to the large receptive fields in deep layers of the backbone, the extracted query and support FG features are inevitably mingled with background (BG) features, impeding the FG-FG matching in cross attention. Hence, the query FG features are fused with less support FG features, i.e., the support information is not well utilized. This paper presents a novel plug-in termed ambiguity elimination network (AENet), which can be plugged into any existing cross attention-based FSS methods. The main idea is to mine discriminative query FG regions to rectify the ambiguous FG features, increasing the proportion of FG information, so as to suppress the negative impacts of the doped BG features. In this way, the FG-FG matching is naturally enhanced. We plug AENet into three baselines CyCTR, SCCAN and HDMNet for evaluation, and their scores are improved by large margins, e.g., the 1-shot performance of SCCAN can be improved by 3.0%+ on both PASCAL-5$^i$ and COCO-20$^i$. The code is available at https://github.com/Sam1224/AENet.

==> sections/sec0_abstract.tex <==
\begin{abstract}
Recent advances in few-shot segmentation (FSS) have built up pixel-pixel matching between query and support features, using cross attention to activate query foreground (FG) with the same-class support FG. However, due to the large receptive field in deep layers of the backbone, the query/support FG features are actually mingled with BG features, impeding the matching process. Although existing methods can learn complex projections to purify the FG features, such operation is class-specific and leads to inductive bias. In this paper, we propose a novel network termed Disc, which can be plugged into any existing cross attention-based baseline to alleviate the issue. The main idea is to mine discriminative query FG regions that are more similar to support FG rather than BG, and aggregate them to the mingled features, thereby increasing the proportion of FG features. In this way, the FG-FG matching is naturally enhanced, and the projections can be relatively simpler. We plug Disc into two baselines (CyCTR and SCCAN) for evaluation, and state-of-the-art performance can be achieved on PASCAL-5$^i$ and COCO-20$^i$, showing the effectiveness of Disc.
\keywords{Few-shot segmentation \and Discriminative query features \and Discriminative prior mask \and Discriminative adaptor}
\end{abstract}

==> sections/sec1_introduction.tex <==
\section{Introduction}
\label{sec:introduction}

% Semantic Segmentation and Few-Shot Segmentation
Semantic segmentation is a dense prediction task in computer vision, which involves assigning each image pixel to the correct class label~\cite{garcia2017review,guo2018review,lateef2019survey}.
The rapid evolution of deep learning techniques has led to significant advancements in semantic segmentation \cite{long2015fully,ronneberger2015u,zhao2017pyramid,chen2017deeplab,zhou2022rethinking}. However, they rely heavily on substantial time and human efforts devoted to the meticulous annotation of pixel-wise masks (\eg, ImageNet~\cite{russakovsky2015imagenet}), and the trained model cannot be directly generalized to novel classes (\ie, unseen classes during training).

To address these challenges, the paradigm of few-shot segmentation (FSS) has been introduced to segment query images containing arbitrary classes, with the help of a few support (image, mask) pairs sharing the same class.
During training, FSS models would learn the class-agnostic pattern on some base classes, enabling it to identify query features resembling support FG~\footnote{FSS belongs to binary segmentation that involves foreground (FG) and background (BG). Query and support FGs share the same class, while the BGs can be different.} features and classify them as query FG. Then, the learned pattern can be directly applied to segment arbitrary novel classes.

% Summary of existing methods
The effectiveness of FSS heavily relies on the skillful utilization of support samples, based on which the existing methods can be categorized into prototype-based~\cite{zhang2019canet,wang2019panet,li2021adaptive,tian2020prior,fan2022self,bao2023relevant,lang2022learning} and cross attention-based methods~\cite{zhang2019pyramid,wang2020few,zhang2021few,wang2022adaptive,xu2023self,peng2023hierarchical}.
Prototype-based methods typically entail the extraction of support prototypes from support FG features, which are subsequently leveraged to segment the query image through feature comparison~\cite{wang2019panet} or concatenation~\cite{tian2020prior}. Nevertheless, the compression of features into prototypes would lead to potential information loss, as well as the disruption of the spatial structure of objects~\cite{xiong2022doubly}. To address these issues, recent advancements in FSS have embraced cross attention~\cite{vaswani2017attention} to fuse query features with the uncompressed support FG features.

\begin{figure}[tb]
  \centering
  \includegraphics[width=1\linewidth]{figures/intro.pdf}
  \caption{Comparisons of (a) existing cross attention-based methods, and (b) our plug-in discriminative adaptor (DA). \textcolor{red}{$\star$} is sampled FG pixel.
  In (a), due to the large receptive field during feature extraction, each FG pixel's features is inevitably fused with BG features, which hinders FG-FG matching. To address it, FSS model can learn to detach \emph{base class-specific} BG features from FG, but it leads to \emph{inductive bias}.
  In (b), discriminative query FG regions are mined and fused with the mingled query/support features, so as to increase the proportion of FG, thus the FG-FG matching is naturally enhanced, \ie, the projections are less likely to get biased.
  }
  \label{fig:intro}
\end{figure}

% Limitations
Despite their success, existing cross attention-based methods overlook the \emph{inductive bias} raised by the \emph{base class-specific projections} in attention mechanism, for which we explain as follows.
(1) \emph{Feature entanglement}: It is a common practice~\cite{shaban2017one,tian2020prior} to forward the query and support images to a pretrained backbone (\eg, VGG-16~\cite{simonyan2014very} or ResNet-50~\cite{he2016deep}) to extract their features. However, deep convolution layers have large receptive field, so each pixel's features are likely to be aggregated with the features from different classes. In this way, semantics like ``a bird resting on the fence'' and ``a bird resting on a man's shoulder'' are formed. A direct evidence is that the query prior mask~\cite{tian2020prior} (\textcolor{red}{Figure ?}) calculated with support BG also have high responses on query FG, especially on border areas;
(2) \emph{Class-specific projections}: To better utilize the support samples, query FG features are expected to be better fused with more support FG features. Take \cref{fig:intro}(a) as an example, the query FG features contain FG (bird) and BG (fence), and support FG features consist of FG (bird) and BG (human). Unfortunately, as their BG classes are different, the doped BG would hinder the similarity-based matching between query and support FGs, \ie, the support information would not be effectively utilized. During training, FSS models can learn complex projections (to obtain $Q$, $K$ and $V$) to detach BGs from FG features, and improve the FG-FG matching. However, each class appears with their own BG classes, so the FSS models tend to learn \emph{base class-specific projections} that cannot be safely applied to novel classes, \ie, they get biased towards base classes, thereby leading to poor performance on novel classes. 

% Solutions
The design principle of this paper is: Discriminative query FG regions can be easily obtained via comparisons, \ie, extract those regions that are more similar to support FG rather than support BG. With this idea, we propose a plug-in network named \textbf{Discriminative (Disc)}, which includes: (1) \textbf{Discriminative prior mask (DPM)}: We devise the learning-agnostic prior masks~\cite{tian2020prior} and generate three prior masks. As illustrated in (\textcolor{red}{Figure ?}), the first two masks display the regions that are similar to the mingled support FG and BG features, respectively, and the third mask is their subtractions, mitigating the issue of feature entanglement. In brief, DPM can accurately locate the query FG regions without additional learnable parameters, and improve the convergence speed;
and (2) \textbf{Discriminative adaptor (DA)}: As shown in \cref{fig:intro}(b), we insert a lightweight DA module before the cross attention block, aiming at purifying the query/support features with some explicit and class-agnostic guidance. In detail, the discriminative query FG regions are mined, and then used to refine the query and support features. For a query FG pixel, its features would consequently contain more FG information, so the FG-FG matching between query and support features is naturally enhanced, and the FSS models can pay less attention to the projections, becoming less likely to get biased. Up to now, the aforementioned issues have been addressed.
In this paper, we validate the effectiveness of Disc on two representative cross attention-based FSS baselines, namely, CyCTR~\cite{zhang2021few} and SCCAN~\cite{xu2023self}.
%
% Contributions
To sum up, our contributions are summarized as follows:
\begin{itemize}
    \item To the best of our knowledge, we are the first to identify the inductive bias raised by the projection operation in cross attention. 
    \item We propose a simple but effective idea to obtain the discriminative query FG regions. Then, we propose the plug-in network Disc to mitigate the aforementioned inductive bias issue for existing cross attention-based FSS methods.
    \item Extensive experiments are conducted on two public benchmark datasets to validate the effectiveness of Disc. Notably, Disc is plugged into CyCTR and SCCAN, and can improve their performance by large margins.
\end{itemize}

==> sections/sec4_methodology.tex <==
\section{Methodology}
\label{sec:methodology}

\begin{figure}[tb]
  \centering
  \includegraphics[width=1\linewidth]{figures/overview.pdf}
  \caption{Overview of the plug-in network Discriminative (Disc). Disc is designed for existing cross attention-based methods such as SCCAN~\cite{xu2023self}. In detail, Disc includes discriminative prior mask (DPM) and discriminative adaptor (DA), sharing the same main idea: To mine those query FG regions that are more similar to support FG, compared to support BG. With such idea, (1) DPM helps to locate the query FG without any learnable parameters; (2) DA mines the most discriminative query FG regions, and then refines the query and support features for boosting FSS.
  }
  \label{fig:overview}
\end{figure}

The standard FSS pipeline is described as follows:
The query image $I_Q$ and the support image $I_S$ are forwarded to a frozen ImageNet-pretrained~\cite{russakovsky2015imagenet} backbone (\eg, VGG16~\cite{simonyan2014very} or ResNet50~\cite{he2016deep}) for extracting their mid-level features $\{F_Q, F_S\}$ (from blocks 2 and 3) and high-level features $\{F_Q^h, F_S^h\}$ (from block 4). As explained in existing methods~\cite{zhang2019canet,tian2020prior}, FSS models would witness severe overfitting phenomena if segmentation is carried out with the high-level features. In spite of this, PFENet~\cite{tian2020prior} demonstrates that learning-agnostic prior masks can be derived from high-level features to coarsely locate the query FG objects and improve the convergence speed. Therefore, almost all recent advances~\cite{lang2022learning,peng2023hierarchical,xu2023self} follow the same guideline to take the mid-level features for segmentation, and use the high-level features for generating prior masks.
Then, support FG features are obtained with $F_S$ and support mask $M_S$, which are fused with query features, either in a prototypical way or a cross attention manner, to activate those query FG that share the same class.
Finally, the enhanced query features are processed by a decoder to obtain the predicted query mask $\hat{M}_Q$.

% % =====
% % incorporate into intro
% % =====
% However, as discussed in ~\cref{sec:introduction}, deep convolution layers of the backbone essentially have large receptive field, so the extracted FG/BG features are also fused with BG/FG features, especially for those pixels locating at the boundary area between FG and BG objects. Some direct evidences are provided in ~\cref{fig:dpm}, \eg, for $M_{Prior}^{FG}$ measured with support FG, many query BG regions are wrongly activated.
% Therefore, when existing methods~\cite{zhang2021few,xu2023self} conduct cross attention on the entangled query features and support FG, (1) the support information is distributed to query FG and many wrongly activated query BG, making the enhanced query FG and BG hard for separation (\ie, segmentation); and (2) as query FG and support BG are doped with different-class BG information, the similarity-based attention score would be relatively smaller, which hinders query FG from fusing more support FG, thereby leading to ineffective FSS.
% The model can naturally address these problems by learning complex projections (in cross attention) to detach the class-specific BG features from the FG features. This works well with the semantic segmentation task, but for FSS, where the novel classes have not been witnessed during training, the model would fail to deal with their unseen BG classes. This issue is known as \emph{inductive bias}.

To mitigate this issue, we present the overview of our plug-in network Discriminative (Disc) in \cref{fig:overview}, whose main components, including the discriminative prior mask (DPM) module (\cref{sec:dpm}) and the discriminative adaptor (DA) module (\cref{sec:da}), can be plugged into any existing cross attention-based FSS baselines such as CyCTR~\cite{zhang2021few} and SCCAN~\cite{xu2023self}. Take SCCAN as an example, its pseudo mask aggregation (PMA) module is replaced with our proposed DPM, and we insert one DA before each self-calibrated cross attention (SCCA) block, with other parts remaining untouched. Particularly, the learning-agnostic DPM can not only approximately locate the query FG, but also extract the most discriminative query FG regions. In this way, the FSS model can obtain some hints with no additional learnable parameters, and its converge speed is well improved. Besides, the DA module aims at using the mined discriminative query FG regions to refine the BG-entangled query and support FG features, so as to better utilize the support samples.

\subsection{Discriminative Prior Mask (DPM)}
\label{sec:dpm}

% \begin{figure}[tb]
%   \centering
%   \includegraphics[width=0.55\linewidth]{figures/dpm_examples.pdf}
%   \caption{TODO
%   }
%   \label{fig:dpm_examples}
% \end{figure}

\begin{figure}[tb]
  \centering
  \includegraphics[width=1\linewidth]{figures/dpm.pdf}
  \caption{Details of the learning-agnostic discriminative prior mask (DPM) module.
  }
  \label{fig:dpm}
\end{figure}

Since PFENet~\cite{tian2020prior}, learning-agnostic prior masks are widely adopted in FSS models~\cite{zhang2021few,xu2023self,peng2023hierarchical}, to coarsely locate the query FG objects and improve the convergence speed. For each query pixel, most of the existing methods~\cite{tian2020prior,liu2022dynamic,luo2021pfenet++,zhang2021few} take its high-level features, calculate its cosine similarity scores with each support FG feature, take the normalized maximum score, showing how likely this query pixel belongs to FG class. Later, SCCAN~\cite{xu2023self} indicates the operation of taking a single maximum score is heavily affected by noises, and they propose to utilize all pairwise similarities for generating more robust prior masks.

Nevertheless, they overlook the fact that the high-level FG and BG features are inevitably fused with BG and FG features (\ie, feature entanglement), which means query-support FG-FG may not consistently have large similarity scores, while query-support BG-FG can also have high scores. Hence, the generated prior masks would be less effective. We prove the claim by providing some direct evidences in \cref{fig:dpm}, where $M_{Prior}^{FG}$ and $M_{Prior}^{BG}$ are the query prior masks calculated with support FG and BG, respectively. We could observe that (1) there are many BG regions wrongly activated in $M_{Prior}^{FG}$, and (2) support BG can also have high responses on query FG in $M_{Prior}^{BG}$.

To tackle the aforementioned issue, we propose to extract the most discriminative query FG regions via a simple subtraction operation between $M_{Prior}^{FG}$ and $M_{Prior}^{BG}$, whose essence is the discriminative query FG should naturally be more similar to support FG than support BG. As shown in \cref{fig:dpm}, the discriminative prior masks $M_{Prior}^{Disc}$ can suppress the unexpected areas well, showing the FG regions that are most dissimilar to the BG.

The details of DPM are presented in \cref{fig:dpm}, and we formally describe DPM as follows. Following existing methods, we take the high-level query features $F_Q^h$ and support features $F_S^h$, as well as the downsampled support mask $M_S$ as inputs. Firstly, the support FG and BG prototypes $P_S^{FG}$ and $P_S^{BG}$ are obtained as follows:
\begin{equation}\label{eq:proto_extraction}
    P_S^{FG} = GAP(F_S^h, M_S), P_S^{BG} = GAP(F_S^h, 1 - M_S)
\end{equation}
where $GAP(\cdot)$ denotes the global average pooling (GAP) operation.
Then, two cosine similarity scores $Sim^{FG} \in [-1, 1]$ and $Sim^{BG} \in [-1, 1]$ are calculated with between flattened query features and the prototypes. They are then normalized and reshaped to obtain the prior masks $M_{Prior}^{FG} \in [0, 1]$ and $M_{Prior}^{BG} \in [0, 1]$ that activate the query regions that are similar to support FG and BG.
% \begin{equation}
%     % Sim^{FG} = Cosine(F_Q^h, P_S^{FG}), Sim^{BG} = Cosine(F_Q^h, P_S^{BG})
%     Sim^{*} = Cosine(F_Q^h, P_S^{*})
% \end{equation}
% \begin{equation}
%     % M_{Prior}^{FG} = Norm(Sim^{FG}), M_{Prior}^{BG} = Norm(Sim^{BG})
%     M_{Prior}^{*} = Norm(Sim^{*})
% \end{equation}
\begin{align}
    Sim^{*} &= Cosine(F_Q^h, P_S^{*}) \;
    \\
    M_{Prior}^{*} &= Norm(Sim^{*})
\end{align}
where superscript $* \in \{FG, BG\}$, $Cosine(\cdot)$ means cosine similarity, $Norm(\cdot)$ is the min-max scaler to normalize the values into $[0, 1]$.
Next, we perform a clipped subtraction to obtain the discriminative prior mask $M_{Prior}^{Disc}$.
\begin{equation}\label{eq:disc_prior}
    M_{Prior}^{Disc} = Clip(M_{Prior}^{FG} - M_{Prior}^{BG})
\end{equation}
where $Clip(\cdot)$ is an operator to set the negative values as zeros. The negative values correspond to those query regions that are more similar to support BG, which is not helpful in FSS.
Finally, we concatenate $M_{Prior}^{FG}$ and $M_{Prior}^{Disc}$ as the final prior mask, providing both the coarse location of query FG and the most discriminative query FG regions.

\subsection{Discriminative Adaptor (DA)}
\label{sec:da}

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.82\linewidth]{figures/da.pdf}
  \caption{Details of discriminative adaptor (DA) module. DA is wrapped by a Transformer block, \ie, the input features would be sequentially processed by layer normalization (LN), DA, LN, and feed-forward network (FFN).
  }
  \label{fig:da}
\end{figure}

To tackle the \emph{inductive bias} raised by \emph{feature entanglement} and \emph{base class-specific projections}, we further design the plug-in DA for existing cross attention-based FSS methods~\cite{zhang2021few,xu2023self}.
As verified in \cref{fig:dpm}, discriminative query FG regions can be easily and consistently extracted, whose features are the most discriminative ones that are dissimilar to support BG. Therefore, we use them to refine the entangled query and support FG features, so the proportion of pure FG information in a FG pixel's entangled features can be naturally increased. As a result, (1) the FG-FG matching between query and support features is enhanced, and the support samples would be better utilized for effective FSS; and (2) the model can focus less on the \emph{base class-specific projections}, as its role is taken by DA, but in a more class-agnostic manner. Hence, the \emph{inductive bias} is well mitigated.

As illustrated in \cref{fig:da}, the mid-level query features $F_Q$  and support features $F_S$ are taken as the inputs. $F_Q$ is processed by two linear layers to obtain the projections $K$ and $V$, while $F_S$ is projected to $Q$. Then, the $Q$ and $K$ are forwarded to the DPM module to obtain the support FG prototype $P_S^{FG}$ and the discriminative prior mask $M^{Disc}$, which is supervised by an auxiliary binary cross entropy (BCE) loss $\mathcal{L}_{aux}$. The procedure can be written as:
% \begin{equation}
%     Q = Linear(F_S), K = Linear(F_Q), V = Linear(F_Q)
% \end{equation}
% \begin{equation}
%     P_S^{FG}, M^{Disc} = DPM(Q, K)
% \end{equation}
% \begin{equation}
%     \mathcal{L}_{aux} = \lambda \cdot BCE(M^{Disc}, M_Q)
% \end{equation}
\begin{align}
    Q = Linear(F_S), K &= Linear(F_Q), V = Linear(F_Q) \;
    \\
    P_S^{FG}, M^{Disc} &= DPM(Q, K) \;
    \\
    \mathcal{L}_{aux} &= \lambda \cdot BCE(M^{Disc}, M_Q) \label{eq:aux_loss}
\end{align}
where $DPM(\cdot)$ means processing the inputs through \cref{eq:proto_extraction} to \cref{eq:disc_prior}, $\mathcal{L}_{aux}$ is utilized during training, $\lambda$ is a constant, $M_Q$ is the labelled query mask.
Then, a matrix multiplication is performed to extract and aggregate the discriminative query features into a prototype $P_Q^{FG}$. Next, the cosine similarity $\alpha$ between $P_S^{FG}$ and $P_Q^{FG}$ is measured, and re-scaled to $[0, 1]$. $\alpha$ is utilized to weighted fuse the prototypes to obtain $P^{FG}$, containing the support FG and the most discriminative query FG features. After that, $P^{FG}$ is expanded and concatenated with the input query and support features $F_Q$ and $F_S$, and processed by a linear layer for feature refinement.
% \begin{equation}
%     P_Q^{FG} = Softmax(M^{Disc}) \otimes V
% \end{equation}
% \begin{equation}
%     \alpha = (Cosine(P_S^{FG}, P_Q^{FG}) + 1) / 2
% \end{equation}
% \begin{equation}
%     P^{FG} = \alpha \cdot P_S^{FG} + (1 - \alpha) \cdot P_Q^{FG}
% \end{equation}
% \begin{equation}
%     F_Q = Linear(F_Q || P^{FG}), F_S = Linear(F_S || P^{FG})
% \end{equation}
\begin{align}
    P_Q^{FG} &= Softmax(M^{Disc}) \otimes V \;
    \\
    \alpha &= (Cosine(P_S^{FG}, P_Q^{FG}) + 1) / 2 \;
    \\
    P^{FG} &= \alpha \cdot P_S^{FG} + (1 - \alpha) \cdot P_Q^{FG} \;
    \\
    F_* &= Linear(F_* || P^{FG})
\end{align}
where $\otimes$ is the matrix multiplication operation, subscript $* \in \{Q, S\}$, $||$ denotes feature concatenation.
Finally, we further wrap DA with an attention block~\cite{vaswani2017attention}, and the refined query and support features are forwarded to existing cross attention blocks~\cite{zhang2021few,xu2023self} for feature matching.

